Traversing Time with Multi-Resolution Gaussian Process State-Space Models

Gaussian Process state-space models capture complex temporal dependencies in a principled manner by placing a Gaussian Process prior on the transition function. These models have a natural interpretation as discretized stochastic differential equations, but inference for long sequences with fast and slow transitions is difficult. Fast transitions need tight discretizations whereas slow transitions require backpropagating the gradients over long subtrajectories. We propose a novel Gaussian process state-space architecture composed of multiple components, each trained on a different resolution, to model effects on different timescales. The combined model allows traversing time on adaptive scales, providing efficient inference for arbitrarily long sequences with complex dynamics. We benchmark our novel method on semi-synthetic data and on an engine modeling task. In both experiments, our approach compares favorably against its state-of-the-art alternatives that operate on a single time-scale only.

==> sections/checklist.tex <==
%!TEX root = ../paper.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{(see Section~\ref{sec:limitations}).}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{(see Supplementary Material ~\ref{sec:appxgpssmOverview} and ~\ref{sec:appxsdeOverview}).}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{(see Supplementary Material ~\ref{sec:appxproof} and ~\ref{appx:sde_proofs}).}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{(We included code, data and instructions to reproduce the experimental results in Section~\ref{sec:toydata} in the supplemental material. After acceptance, we will make all information needed to reproduce Section~\ref{sec:toydata} and ~\ref{sec:engine} available on GitHub).}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{(see Section~\ref{sec:experiments} and Supplementary Matrial~\ref{sec:appxexperiments}).}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{(see Section~\ref{sec:experiments} and Supplementary Matrial~\ref{sec:appxexperiments}).}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{(We provide runtime estimates in Supplementary Table~\ref{table:batchsizeVSresolution}).}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{(We build on existing code as described in Section~\ref{sec:experiments}).}
  \item Did you mention the license of the assets?
    \answerYes{(see Section~\ref{sec:experiments}).}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{(We will make the engine dataset publicly available on GitHub after publication).}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{(see Section~\ref{sec:experiments}).}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{(see Section~\ref{sec:experiments}).}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/inference.tex <==
%\section{Inference} 
%In the first part of this section we give a short recap of stochastic differential equations (SDEs) and the connection between their discretized form and state-space models. The second part analyses how the discretization level of the SDE impacts the the evidence lower bound $\mathcal{L}$ and is also our first technical contribution.

\newpage
\section{Leftovers}

\subsubsection{Regular Sampling}

We choose to use snippets of fixed length, but learn which snippet length to choose.B
\results{Implementation is working. Results are shown in Section~\ref{sec:experiments} using a grid-search over $\delta$.}

\subsubsection{Irregular Sampling}
\label{sec:irregular}
    We choose to not use snippets of fixed length, but irregularly subsample the data $x_{t_1}, \cdots , x_{t_K}$ and employ a varying step size $\Delta_t^k$. If adjacent time points $t_k$ and $t_{k+1}$ are far from each other, we apply a large step size $\Delta_{t_k}$, if they are close to each other,we apply a small step size $\Delta_{t_k}$. This allows us to learn small and large scale effects simulateneously.

\results{
We did not achieve good results with the irregular sampling approach. We think this is due to the following reasons:
Our implementation requires a reference delta that is used to scale the parameters. Depending on how we set this parameter, we run into the following problems:

\begin{itemize}
\item 	
If the reference delta is small, the variance term for the larger deltas increases and it is difficult to learn/ predict.
\item 	
If the reference delta is large, the latent state will probably not converge within one mini-batch because the mean steps are not large enough.
\end{itemize}

}



\open{
\begin{itemize}
    \item 
    Is there one best $\delta$ for each region?
    \item 
    Simulation with different $\delta$ / Pre-Segmentation/ Learn a function on how $\delta$ evolves?
\end{itemize}
}

\subsubsection{Stacked Models} 
\label{sec:stacked}
We learn multiple models at different resolutions by down-sampling the data by factor $d$ and using as step size $\Delta_t = d$. 
%After learning the model, we need to upscale the predictions. We can achieve this by changing the step size to $\Delta_t = 1$. The predicted outputs of the lower resolution models are then incorporated as additional inputs to the models of higher resolution.

\paragraph{Separate Learning}

We present three different strategies for stacking the models, where each model is learnt independently from the others:
\begin{enumerate}
    \item Residual Learning
    \item Previous prediction as a feature for the next model
    \item Previous prediction as a mean for the next model
\end{enumerate}
With all the models we start we the lowest resolution model, i.e the one with the largest delta.

In residual learning, we train the first model $M1: (x_0,y_0)$ with the lowest resolution data $f_0$, and then use $M1$ to predict $y$ on the next higher resolution $f_1$. The residual is defined as $y - f$, and the next model is trained using the residual as output $M2 : (x_1, y_1-f_1)$.

In option two, we give the prediction on the lower resolution model $M1 : (x_0, y_0)$ as an input for the next higher resolution model $M2 : ((x_1, pred_0), y_1)$.

In the last strategy, we give the prediction on the previous model as a mean for the next model. That is, in the emission model we sum the prediction form previous model to the predicted $y:s$ of the current model: $y_1 = y_1 + \alpha pred_0$. We also introduce a scaling variable $\alpha$ to allow learning how relevant the previous model has been.

\results{All the options have been implemented and are working. They improve the results at least on one data set, though in some other data sets no effect was observed. Results are shown in Section 5. Variance in the results is not meaningful currently. These work as a baseline for now while we attempt to get a working implementation with joint learning.}
%
%\section{Derivation of the ELBO}
%\label{appx:elbo}
%
%\begin{small}
%
%\begin{eqnarray}
%%\begin{align*}
%\log p\left(\boldsymbol{y}_{1: T}\right) \geq & \mathbb{E}_{q\left(\boldsymbol{x}_{1: T}, \boldsymbol{f}_{2: T}, \boldsymbol{z}\right)}\left[\log \frac{p\left(\boldsymbol{y}_{1: T}, \boldsymbol{x}_{1: T}, \boldsymbol{f}_{2: T}, \boldsymbol{z}\right)}{q\left(\boldsymbol{x}_{1: T}, \boldsymbol{f}_{2: T}, \boldsymbol{z}\right)}\right] \\
%=&\mathbb{E}_{q\left(\boldsymbol{x}_{1: T}, f_{2: T}, \boldsymbol{z}\right)}\left[\log \frac{\left[\prod_{t=1}^{T} p\left(\boldsymbol{y}_{t} \mid \boldsymbol{x}_{t}\right)\right]\left[\prod_{t=2}^{T} p\left(\boldsymbol{x}_{t} \mid \boldsymbol{f}_{t}\right)\right]\left[\prod_{t=2}^{T} \prod_{d=1}^{D_{x}} p\left(f_{t, d} \mid \hat{\boldsymbol{x}}_{t-1}, \boldsymbol{z}_{d}\right) p\left(\boldsymbol{z}_{d}\right)\right] p\left(\boldsymbol{x}_{1}\right)}{\left[\prod_{t=2}^{T} p\left(\boldsymbol{x}_{t} \mid \boldsymbol{f}_{t}\right)\right]\left[\prod_{t=2}^{T} \prod_{d=1}^{D_{x}} p\left(f_{t, d} \mid \hat{\boldsymbol{x}}_{t-1}, \boldsymbol{z}_{d}\right) q\left(\boldsymbol{z}_{d}\right)\right] q\left(\boldsymbol{x}_{1}\right)}\right] \\
%=&\mathbb{E}_{q\left(\boldsymbol{x}_{1: T}, \boldsymbol{f}_{2: T}, \boldsymbol{z}\right)}\left[\log \frac{\left[\prod_{t=1}^{T} p\left(\boldsymbol{y}_{t} \mid \boldsymbol{x}_{t}\right)\right]\left[\prod_{d=1}^{D_{x}} p\left(\boldsymbol{z}_{d}\right)\right] p\left(\boldsymbol{x}_{1}\right)}{\left[\prod_{d=1}^{D_{x}} q\left(\boldsymbol{z}_{d}\right)\right] q\left(\boldsymbol{x}_{1}\right)}\right]\\
%=&\mathbb{E}_{q\left(\boldsymbol{x}_{1: T}, \boldsymbol{f}_{2: T}, \boldsymbol{z}\right)}\left[\log \prod_{t=1}^{T} p\left(\boldsymbol{y}_{t} \mid \boldsymbol{x}_{t}\right)\right]+\mathbb{E}_{q\left(\boldsymbol{x}_{1: T}, \boldsymbol{f}_{2: T}, \boldsymbol{z}\right)}\left[\sum_{d=1}^{D_{x}} \log \frac{p\left(\boldsymbol{z}_{d}\right)}{q\left(\boldsymbol{z}_{d}\right)}\right]+\mathbb{E}_{q\left(\boldsymbol{x}_{1: T}, \boldsymbol{f}_{2: T}, \boldsymbol{z}\right)}\left[\log \frac{p\left(\boldsymbol{x}_{1}\right)}{q\left(\boldsymbol{x}_{1}\right)}\right] \\
%=&\mathbb{E}_{q\left(\boldsymbol{x}_{1: T}\right)}\left[\log \prod_{t=1}^{T} p\left(\boldsymbol{y}_{t} \mid \boldsymbol{x}_{t}\right)\right]+\mathbb{E}_{q(\boldsymbol{z})}\left[\sum_{d=1}^{D_{x}} \log \frac{p\left(\boldsymbol{z}_{d}\right)}{q\left(\boldsymbol{z}_{d}\right)}\right]+\mathbb{E}_{q\left(\boldsymbol{x}_{1}\right)}\left[\log \frac{p\left(\boldsymbol{x}_{1}\right)}{q\left(\boldsymbol{x}_{1}\right)}\right] \\
%=&\sum_{t=1}^{T} \mathbb{E}_{q\left(\boldsymbol{x}_{t}\right)}\left[\log p\left(\boldsymbol{y}_{t} \mid \boldsymbol{x}_{t}\right)\right]+\sum_{d=1}^{D_{x}} \operatorname{KL}\left(q\left(\boldsymbol{z}_{d}\right) \| p\left(\boldsymbol{z}_{d}\right)\right)+\operatorname{KL}\left(q\left(\boldsymbol{x}_{1}\right) \| p\left(\boldsymbol{x}_{1}\right)\right)
%%\end{align*}
%\end{eqnarray}
%\end{small}

\subsubsection{Joint Learning}
\begin{itemize}
\item Backfitting Algorithm
    \item 
    Initialize all components with zero:
    $g^{(l)} (x) = 0$
    \item 
    Fot $n=1, \ldots N$ do 
    
    For $l = L, \ldots, 1$ do
    
    fitComponent  $g^{(l)} (x)$ on $y - \sum_{l'}g^{(l')} (x)$
    
    end
    
    end
    \item 
    boosting
    \item 
    window sizes vs. time vs. accuracy
    \item 
    stacking vs. joint (variance)
    \item 
    alternative: leight-weight backpropagation of the variance? (only update the variance in the second iteration)
    
\end{itemize}

What we want 
$
\mathcal{N} (y \vert f(x) +  g(x), \sigma^2)
$

Residual Learning
%\begin{itemize} 
$
\mathcal{N} (y \vert f(x) +  g(x), \sigma^2) = \mathcal{N} (y  - g(x) \vert f(x) , \sigma^2)
$
%\end{itemize}

Mean Residual Learning
%\begin{itemize} 
$
\mathcal{N} (y \vert f(x) +  \alpha g(x), \sigma^2)
$
%\end{itemize}


%\paragraph{Joint Learning}
%
%
%\begin{itemize}
%    \item 
%    	Warm start the latent state of the first model by using the coarse discretization level  $\delta_1$ for k time steps
%\item 	
%Warm start the latent state of the next model i by using the discretization level $\delta_i$ for k time step 
%\item 
%When all models are warm started, evaluate the log-likelihood for k time steps
%
%\end{itemize}
%
%\subsection{Algorithmic Choices}
%First, we discuss how to come up with implementation for the first two strategies, i.e. regular sampling~\ref{sec:regular} and irregular sampling~\ref{sec:irregular}. Both can be casted into hyperparameter optimization problems as we outline in the following.
%
%\begin{itemize}
%    \item 
%For regular sampling, the hyperparameter we want to tune is the fixed step size $\Delta_t$.
%\item 
%For irregular sampling, we fix a-priori a set of potential step sizes (for instance $\Delta_t \in \{1, 10, 100 \}$ and use hyperparameter optimization to learn the probability with which each step size is selected.
%\end{itemize}
%
%For both tasks, we use a validation set to find the best hyperparameter configuration. 
%In the following, we will give a brief and non-exhaustive overview of existing algorithms for hyperparameter optimization:
%
%\begin{itemize} 
%\item Grid Search/ Random Search~\citep{bergstra2012random}: 
%Train $l$ models from scratch (can be parallelized). Select best one.
%\item 
%Hyperband~\citep{li2017hyperband}: Grid-search but with early stopping for bad runs. Can be parallelized.
%\item 
%Population-based training~\citep{jaderberg2017population}:
%Keep a population of a small number of models.
%After a fixed number of iterations, compare the models and discard the worst ones and copy over the best-performing methods (exploit phase). 
%Perturb the parameters of the copied-over models (explore phase).
%\item Bayesian Optimization~\citep{snoek2012practical}: 
%Train $l$ models sequentially. Naive version requires full training of each model. Extensions exist.
%\item 
%Hypergradients~\citep{lorraine2020optimizing}:
%Not straight-forward to obtain gradients of the hyperparameters with respect to the validation set. Active field of research.
%\end{itemize}
%
%We opted for grid-search since the focuss of our paper will most likely be rather the stacked modeling approach.


%\subsubsection{Variance Prediction}
%$$ (\Sigma_1(x_t) + \sigma_1^2) \cdot 1 = (\Sigma_{k}(x_t) + \sigma_{k}^2) \cdot k $$ 
%$$ (K^1_{t, t}-K^1_{t, 1: t-1}(K^1_{1: t-1,1: t-1}+\sigma_1^{2} {I})^{-1} K^1_{1: t-1, t} ) \cdot 1 =  (K^k_{t, t}-K^k_{t, 1: t-1}(K^k_{1: t-1,1: t-1}+\sigma_k^{2} {I})^{-1} K^k_{1: t-1, t} ) \cdot k $$

%What must be fulfilled?
%$$ K^1_{t, t} \cdot 1 = K^k_{t, t} \cdot k$$
%$$ \alpha^2_1 \exp(-d^2/l) \cdot 1 = \alpha^2_k \exp(-d^2/l) \cdot k $$
%$$ \alpha^2_1 = \alpha^2_k \cdot k$$

%Which else parameteres to consider?
%\begin{itemize}
%\item noise level $\sigma^2$
%\item variational parameters (mean and covariance)
%\end{itemize}

\subsection{Diluted Mini-Batching}
The goal of this section is to extend the mini-batch scheme of Eq.~\eqref{eq:elbo_mbs} to diluted minibatches of factor $N$, 
\begin{align}
\mathcal{L} \approx
&
-  \operatorname{KL}\left(q\left(X_{0}\right) \|
p\left(X_{0} \right)\right)
-
%- \sum_{t=1}^T \mathbb{E}_{q\left({x}_{t-1}\right)}\left[
%\kappa(x_{t-1})
%\right]
 \operatorname{KL}\left(q\left({F}^l_{M}\right) \| p\left({F}^l_{M} \right)\right)
\nonumber
\\
&
+ \sum_{s=1}^S \mathbb{E}_{q\left({X}_{t_0 + s N  }\right)}\left[\log p\left({y}_{t_0 + s N} \mid {X}_{t_0 + s N_l}\right)\right],
%- \sum_{t=1}^T \mathbb{E}_{q\left({x}_{t-1}\right)}\left[
%\kappa(x_{t-1})
%\right]
\label{eq:elbo_diluted}
\end{align}
 without increasing the runtime or memory burden. 
This allows us to pack a longer history into one mini-batch which is needed to capture effects with slow dynamics.

To do so, we interpret the approximate posterior over the latent state, $q(x^l_{t+1} \vert \mu_t^l, \Sigma_t^l, + Q^l)$, as the Euler Maruyama approximation of the SDE which drift term is specified by the GP mean predictions $\bar{f}(x^l_t) := \mu^l_t$ and which diffusion term is specified by the noise GP variance predictions $\bar{L}^l = \sqrt{\Sigma^l_t + Q^l}$.

To sample efficiently from the marginal $q\left({X}_{t_0 + s N_l   }\right)$ we need to make a second approximation t

The second approximation is more interesting and has to our knowledge not been done before:
To sample efficiently from $q(X_{t+N} \vert X_t, f_M)$, we connect our state-space model with stochastic differential equations to apply the Euler-Maruyama scheme [Eq.~\eqref{eq:em}]:
\begin{align}
{X}_{t + N}  &\sim q({X}_{t + N} \vert  {X}_{t }, f_M)
\nonumber \\
&=
\int   \prod_{n=1}^N q({X}_{t + n} \vert  {X}_{t+n-1}, f_M) df_M dX_{t+1, \ldots, t+N-1},
\nonumber \\
&\approx \prod_l
\mathcal{N}(x^l_{t+N} \vert x^l_t + N \mu^l_t, N(Q^l + \Sigma^l_t)).
\end{align}
Instead of sampling $N$ times with the approximate posterior over one time step, we sample one time with the larger step size $N$.



\paragraph{Impact of Stepsize on the Evidence Lower Bound $\mathcal{L}$}
\label{sec:sde_elbo}

We define
$K_{MM}= \frac{1}{\Delta_t} K^0_{MM}$, $\sigma^2 = \frac{1}{\Delta_t} \sigma_0^2$, $\mu_M = \frac{1}{\Delta_t} \mu^0_M $ and $ \Sigma_M= \frac{1}{\Delta_t} \Sigma_M^0$, where $K^0_{MM}$,$\sigma_0^2$, $\mu_M^0$ and $\Sigma_M^0$ correspond to the values when $\Delta_t = 1$.
We have defined
\begin{equation}
\begin{aligned}
%q(z) =& \mathcal{N}(z_M|\mu_M,\Sigma_M) \\
x_{t+1} \sim& q(x_{t+1}|x_t) = N(x_{t+1}| x_t + \mu(x_t) \Delta_t, \Sigma(x_t)  \Delta(t)) 
\label{eq:q_x}
%\mu(x) =& K_{nm}K_{mm}^{-1} m \\
%\Sigma(x) =& K_{nm} - K_{nm}K_{mm}^{-1}K_{mn} + K_{nm}K_{mm}^{-1}QK_{mm}^{-1}K_{mn} \\
%\log p(\boldsymbol{y}_{1: T})=&\sum_{t=1}^{T} \mathbb{E}_{q(\boldsymbol{x}_{t})}[\log p(\boldsymbol{y}_{t} | \boldsymbol{x}_{t})]+\sum_{d=1}^{D_{x}} \operatorname{KL}(q(\boldsymbol{z}_{d}) \| p(\boldsymbol{z}_{d})))
\end{aligned}
\end{equation}
where $\mu(x_t)$ and $\Sigma(x_t)$ follow Eqs.~\eqref{eq:sgp_mean},\eqref{eq:sgp_cov}.
We first reformulate the approximate posterior $q(x_t)$ [Eq.\eqref{eq:q_x}]  as
%Now we can write the first term in the ELBO as
\begin{equation*}
\begin{aligned}
    \mathcal{N}(x_{t+1} |& x_t + (\frac{1}{\Delta_t}K_{tM}^0 (\frac{1}{\Delta_t}K_{MM}^0)^{-1} \frac{1}{\Delta_t}\mu_M^0) \Delta_t, \\ &[\frac{1}{\Delta_t}K_{tM}^0 - \frac{1}{\Delta_t}K_{tM}^0(\frac{1}{\Delta_t}{K_{MM}}^0)^{-1}\frac{1}{\Delta_t}K_{Mt}^0 \\
    &+ \frac{1}{\Delta_t}K_{tM}^0(\frac{1}{\Delta_t}K_{MM}^0)^{-1}\frac{1}{\Delta_t}\Sigma_M^0(\frac{1}{\Delta_t}K_{MM}^0)^{-1}\frac{1}{\Delta_t}K_{Mt}^0]\Delta_t) \\
    =&  \mathcal{N}(x_{t+1} | x_t + (K_{tM}^0 (K_{MM}^0)^{-1} \mu_M^0), \\ &[K_{tM}^0 - K_{tM}^0(K_{MM}^0)^{-1}K_{Mt}^0\\
    &+ K_{tM}^0(K_{MM}^0)^{-1} \Sigma_M^0(K_{MM}^0)^{-1}K_{Mt}^0]
    \\
    =&
    \mathcal{N}(x_{t+1} \vert 
    x_t+ \mu_0(x_t),
    \Sigma_0(x_t))
\end{aligned}
\end{equation*} 
Since $\log p(y_t \vert x_t)$ is independent of $\Delta_t$, we conclude that the first term of the ELBO is independent of $\Delta_t$.
The second term can be rewritten as
\begin{equation*}
\begin{aligned}
    \KL(q(z_M)||p(z_M)) =& \KL(\mathcal{N}(z_M|\mu_M,\Sigma_M)||\mathcal{N}(z_M|0,K_{MM})) \\
  %  =& \frac{1}{2} \left[
   % \tr\left({\Delta_t}{\left(K_{MM}\right)^0}^{-1}\frac{1}{\Delta_t}\Sigma_M^0\right) \\
   % &+ \frac{1}{\Delta_t} {\mu_M^0}^T \left(
    %\frac1{\Delta_t} K_{MM}^0\right)^{-1}\frac{1}{\Delta_t}\mu_M^0 
   % \\
   % &
   % + \ln \lvert \frac{1}{\Delta_t}K_{MM}^0 \rvert  - \ln \lvert \frac{1}{\Delta_t}\Sigma_M^0 \rvert ) \right] \\
   % =& \frac{1}{2} \left[\tr\left( \left(K_{MM}^0\right)^{-1}\Sigma_M^0 \right) + \frac{1}{\Delta_t} {\mu_M^0}^T \left( K_{MM}^0\right)^{-1}}\mu_M^0 \\
   % &+ \ln\lvert K_{MM}^0 \rvert - \ln\lvert \Sigma_{MM}^0 \rvert)
   % \right]
    \\
    =&
    \KL(\mathcal{N}(z_M \vert \mu_M^0, \Sigma_M^0 \Vert \mathcal{N}(z_M \vert 0, K^0_{MM}) \\
    &- \frac12 \left( 1 - \frac{1}{\Delta_t} \right)
    {\mu_M^0}^\top \left(K_{MM}^0\right)^{-1} \mu_M^0
\end{aligned}
\end{equation*}
which reveals that the KL-divergence is not independent of $\Delta_t$.


\subsection{Sampling Scheme}
which in turn requires sampling the inducing outputs $f_M$ (see Appx.~\ref{appx:elbo}, \citet{ialongo2019overcoming}). Since the latter act as global latent variables, this step can slow down convergence~\cite{kingma2015variational, lindinger2020beyond}.
In contrast, \citet{doerr2018probabilistic} replace $q(x_t\vert x_{t-1}, f_M)$ by $\tilde{q}(x_t \vert x_{t-1}) =  \int q(x_t \vert x_{t-1}, f_M) q(f_M) df_M$, which allows marginalizing out the inducing outputs, i.e. $\tilde{q}(x_t\vert x_{t-1}) =  \mathcal{N}(x_t \vert A_t \tilde{\mu}_t + b_t, S_t + A_t \tilde{\Sigma_t} A_t^\top)$ with 
\begin{align}
\tilde{\mu}^d_t &=K_{tM}K_{MM}^{-1} m^d_M,
\label{eq:sgp_mean}
\\
\tilde{\Sigma}^d_t &=K_{t t}-K_{t M}K_{MM}^{-1}\left(
K_{MM} - S^d_M
\right)
K_{MM}^{-1} K_{Mt}
\label{eq:sgp_cov},
\end{align}
but leads to a biased estimate of the lower bound $\mathcal{L}$ [Eq.~\eqref{eq:elbo2}].

\subsection{Motivating Example}
We begin by giving a motivating example with generated data. We simulated data from the noisy pendelum model using Euler’s discretization with a small step size. We then created noisy observations and used mini-batches of size 100. As we can not see much in one minibatch in the original data, it should not be possible to learn the dynamics using such minibatches. This is a clear example of a data set where downsampling the original dataset will be helpful for learning. See Figure \ref{fig:pendelumdata} for visual illustrations of the data.

\begin{figure*}[h]
\centering
\includegraphics[width=0.7\textwidth]{figures/pendelum.png}
\caption{Simulated data from the noisy pendelum model. The position and velocity are shown in upper plots. When splitting the original data set into minibatches of size 100, we can not see much changes in the data in one batch (bottom left). However, if we downsample the data by a factor of 30, the effects are visible in the minibatches (bottom right).}
\label{fig:pendelumdata}
\end{figure*}


We experimentally confirm the assumption and the results are shown in Figure \ref{fig:pendelumresults}. Here we use minibatches of size 40 and a constant input $u_t = 0$. When using $\Delta_t = 1$ we are not able to learn anything. However, with $\Delta_t = 30$, we can approximately learn the original data set both in training and test data and both with downscaled and upscaled resolution.


\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth]{figures/generated_delta=30.pdf}
\caption{Results on the simulated data from the noisy pendelum model.}
\label{fig:pendelumresults}
\end{figure*}



